Distributionally Robust Policy and Lyapunov-Certificate Learning

This article presents novel methods for synthesizing distributionally robust stabilizing neural controllers and certificates for control systems under model uncertainty. A key challenge in designing controllers with stability guarantees for uncertain systems is the accurate determination of and adaptation to shifts in model parametric uncertainty during online deployment. We tackle this with a novel distributionally robust formulation of the Lyapunov derivative chance constraint ensuring a monotonic decrease of the Lyapunov certificate. To avoid the computational complexity involved in dealing with the space of probability measures, we identify a sufficient condition in the form of deterministic convex constraints that ensures the Lyapunov derivative constraint is satisfied. We integrate this condition into a loss function for training a neural network-based controller and show that, for the resulting closed-loop system, the global asymptotic stability of its equilibrium can be certified with high confidence, even with Out-of-Distribution (OoD) model uncertainties. To demonstrate the efficacy and efficiency of the proposed methodology, we compare it with an uncertainty-agnostic baseline approach and several reinforcement learning approaches in two control problems in simulation.

==> computation-graph.tex <==
\begin{tikzpicture}
\providecommand{\bfx}{\mathbf{x}}
\providecommand{\Lie}{\mathcal{L}}
\providecommand{\grad}{\nabla}
\providecommand{\GP}{GP}
\providecommand{\ubfu}{\underline{\mathbf{u}}}
\node [] (gh) {$\grad_\bfx h(\bfx)$};

\node [right=of gh] (L1) {$\underbrace{\grad_\bfx h(\bfx)^\top f(\bfx)}_{\Lie_f h(\bfx)}$};

\path [->,color=red] (gh)  edge [above] node {$[\cdot]$} (L1);

\node [below=of L1] (f1) {$f(\bfx) \sim \GP $};

\path [->,color=red] (f1)  edge [left] node {$[\cdot]$} (L1);

\node [right=of L1] (gL1) {$\grad_\bfx \Lie_f h(\bfx)$};

\path [->,color=blue] (L1)  edge [above] node {$\grad_\bfx$} (gL1);

\node [right=of gL1] (L2) {$\grad_\bfx[\Lie_f h(\bfx)]^\top F(\bfx) \ubfu$};

\node [below=38pt of L2] (f2) {$F(\bfx)\ubfu \sim \GP $};

\path [->,color=red] 
(f2) edge 
    node[above] {$[\cdot]$}
    node[below] {$\ubfu = [1, \mathbf{0}^\top_m]^\top$} 
 (f1);

\path [->,color=red] (f2)  edge [left] node {$[\cdot]$} (L2);

\path [->,color=red] (gL1)  edge [above] node {$[\cdot]$} (L2);

%\node [right=of L2] (gL2) {};
%\draw[dotted] (L2) -- (gL2) ;
%\path[clip] (gh.north west) rectangle (f2.south east); 
\end{tikzpicture}



==> tex/Notation.tex <==
\section{Notations}
\label{sec: notations}

The sets of real, non-negative real, and natural numbers are denoted by $\bbR$, $\bbR_{\geq 0}$, and $\bbN$, respectively. For $N \in \bbN$, we write $[N] := \{1,2, \dots N\}$. 
We use $\boldsymbol{0}_n$ to denote the $n$-dimensional zero vector. 
For scalar $x$, we write $(x)_+ := \max(x,0)$. We denote by $\bfI_n \in \bbR^{n \times n}$ the identity matrix. For a vector $\bfx$, we use $\|\bfx\|$ to denote the Euclidean norm. 
% We use $\text{vec}(\bfX) \in \mathbb{R}^{nm}$ to denote the vectorization of $\bfX \in \mathbb{R}^{n \times m}$, obtained by stacking its columns. 
The gradient of a differentiable function $V$ is denoted by $\nabla V$, while its Lie derivative along a vector field $f$ by $\calL_f V  = \nabla V \cdot f$. A continuous function $\alpha_V: [0,a)\rightarrow [0,\infty )$ is of class $\calK$ if it is strictly increasing and $\alpha_V(0) = 0$. 
We consider a complete separable metric space $\Xi$ with metric $d$, associated with a Borel $\sigma$-algebra $\calF$. The set of Borel probability measures on $\Xi$ is denoted as $\calP(\Xi)$. For a random variable $\bfxi$ with some distribution supported on $\Xi$, we denote the distribution and expectation by $\mathbb{P}^*$ and $\bbE_{\bbP^*}(\bfxi)$, respectively.
